Revising SA-CCR

From SA-CCR to RSA-CCR: making SA-CCR self-consistent and appropriately risk-sensitive by cashflow decomposition in a 3-Factor Gaussian Market Model

==> figures/payreceiveabs.tex <==
\begin{tabular}{p{2.6cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
\toprule
                                        Unnamed: 0 & HW2F Model Numerix &   Unnamed: 2 & Full Approach &   Unnamed: 4 & Full Approach with Discount 1 &   Unnamed: 6 \\
\midrule
                                        Instrument &                Pay &      Receive &           Pay &      Receive &                           Pay &      Receive \\
                                   ATM Swap=Swap A &        3903698.924 &  3668881.042 &    3705132.79 &  3517421.957 &                   3984398.134 &    3796687.3 \\
                   Series of FRA Replcating Swap A &        3903698.924 &  3668881.042 &    3705132.79 &  3517421.957 &                   3984398.134 &    3796687.3 \\
                   Swap A net of replicating  FRAs &                  0 &            0 &             0 &            0 &                             0 &            0 \\
   Forward start 3-10 +swap 3 y replicating Swap A &        3903698.924 &  3668881.042 &    3705132.79 &  3517421.957 &                   3984398.134 &    3796687.3 \\
                                       ATM+100 bps &        4271792.239 &  3707916.853 &   4081349.072 &  3521127.867 &                   4379311.487 &  3819090.282 \\
                                        ATM+500bps &        5778184.114 &  3898078.713 &   5657394.052 &  3607131.361 &                   6025342.132 &   3975079.44 \\
                                        ATM-100bps &         3539967.75 &  3634569.335 &   3338411.251 &  3523210.789 &                   3598384.612 &   3783184.15 \\
                                        ATM-500bps &        2166836.654 &  3577668.148 &   2002316.179 &  3677157.202 &                   2178422.029 &  3853263.052 \\
     Amortising 10 y, 100 mios, 5y 200 mios=Swap A &        6083964.561 &  5640346.835 &   5896264.479 &  5520842.812 &                   6271442.805 &  5896021.138 \\
 200 mios swap 5y, 100 mios forward start 5y-10... &        6083964.561 &  5640346.835 &   5896264.479 &  5520842.812 &                   6271442.805 &  5896021.138 \\
   100mios 10 yr swap, 100 mios 5 year swap=Swap C &        6083964.561 &  5640346.835 &   5896264.479 &  5520842.812 &                   6271442.805 &  5896021.138 \\
 Combinations of FRAs for whole maturity replic... &        6083964.561 &  5640346.835 &   5896264.479 &  5520842.812 &                   6271442.805 &  5896021.138 \\
  Swap A minus swap with average notional 150 mios &        309963.4539 &  217817.1657 &   342640.9517 &  248785.5348 &                   302120.4339 &   208265.017 \\
                              Fwd Start ATM 1y-10y &        3737350.146 &  3691417.507 &   3569398.947 &  3569398.947 &                   3897277.706 &  3897277.706 \\
                    Fwd Start ATM 1y-10y  +100 bps &        3932089.506 &  3931231.189 &    3780612.98 &   3780612.98 &                    4134384.36 &   4134384.36 \\
                    Fwd Start ATM 1y-10y  +500 bps &          4712042.7 &  4891492.864 &   4631071.683 &  4631071.683 &                    5089083.56 &   5089083.56 \\
                    Fwd Start ATM 1y-10y  -100 bps &        3542763.306 &   3451756.35 &   3358956.976 &  3358956.976 &                   3661042.549 &  3661042.549 \\
                    Fwd Start ATM 1y-10y  -500 bps &        2766728.693 &   2495424.52 &   2528757.051 &  2528757.051 &                   2729333.991 &  2729333.991 \\
                             Zero Coupon ATM 20 yr &         3979045.25 &  3933823.656 &   3897236.895 &  3897236.895 &                   4583414.613 &  4583414.613 \\
                      Zero Coupon ATM+100bps 20 yr &        4297831.909 &  4293269.979 &   4232287.451 &  4232287.451 &                   4977456.765 &  4977456.765 \\
                      Zero Coupon ATM+200bps 20 yr &        4616689.976 &   4652787.71 &   4567338.007 &  4567338.007 &                   5371498.918 &  5371498.918 \\
                      Zero Coupon ATM-100bps 20 yr &        3660345.426 &   3574464.17 &   3562186.338 &  3562186.338 &                    4189372.46 &   4189372.46 \\
                      Zero Coupon ATM-200bps 20 yr &        3252587.924 &  3114662.309 &   3133321.627 &  3133321.627 &                   3684998.505 &  3684998.505 \\
\bottomrule
\end{tabular}



==> figures/payreceivepercentdifference.tex <==
\begin{tabular}{p{2.6cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
\toprule
                                        Unnamed: 0 & Full Approach &    Unnamed: 2 & Full Approach with Discount 1 &    Unnamed: 4 &       Current &    Unnamed: 6 \\
\midrule
                                        Instrument &           Pay &       Receive &                           Pay &       Receive &           Pay &       Receive \\
                                   ATM Swap=Swap A &   -0.05086615 &  -0.041282092 &                   0.020672498 &   0.034835214 &   0.007939772 &   0.072450526 \\
                   Series of FRA Replcating Swap A &   -0.05086615 &  -0.041282092 &                   0.020672498 &   0.034835214 &  -0.102825432 &  -0.045403937 \\
                   Swap A net of replicating  FRAs &             0 &             0 &                             0 &             0 &           NaN &           NaN \\
   Forward start 3-10 +swap 3 y replicating Swap A &   -0.05086615 &  -0.041282092 &                   0.020672498 &   0.034835214 &   -0.06376128 &  -0.003839579 \\
                                       ATM+100 bps &  -0.044581561 &  -0.050375721 &                   0.025169587 &   0.029982719 &  -0.078912741 &   0.061160096 \\
                                        ATM+500bps &  -0.020904502 &  -0.074638655 &                   0.042774341 &   0.019753508 &  -0.319043263 &   0.009393009 \\
                                        ATM-100bps &  -0.056937383 &  -0.030638718 &                   0.016502089 &    0.04088925 &   0.111505438 &   0.082574864 \\
                                        ATM-500bps &   -0.07592657 &   0.027808352 &                   0.005346676 &   0.077031992 &   0.815869874 &   0.099792725 \\
     Amortising 10 y, 100 mios, 5y 200 mios=Swap A &  -0.030851607 &  -0.021187354 &                   0.030815144 &   0.045329536 &  -0.029902287 &   0.046396663 \\
 200 mios swap 5y, 100 mios forward start 5y-10... &  -0.030851607 &  -0.021187354 &                   0.030815144 &   0.045329536 &  -0.052800709 &   0.021697262 \\
   100mios 10 yr swap, 100 mios 5 year swap=Swap C &  -0.030851607 &  -0.021187354 &                   0.030815144 &   0.045329536 &  -0.062107418 &   0.011658573 \\
 Combinations of FRAs for whole maturity replic... &  -0.030851607 &  -0.021187354 &                   0.030815144 &   0.045329536 &  -0.095580196 &  -0.024446865 \\
  Swap A minus swap with average notional 150 mios &   0.105423711 &   0.142175981 &                  -0.025303048 &  -0.043853975 &            -1 &            -1 \\
                              Fwd Start ATM 1y-10y &  -0.044938577 &  -0.033054662 &                   0.042791698 &   0.055767249 &   0.001457181 &   0.013918402 \\
                    Fwd Start ATM 1y-10y  +100 bps &  -0.038523163 &  -0.038313241 &                   0.051447164 &   0.051676729 &  -0.048140655 &  -0.047932833 \\
                    Fwd Start ATM 1y-10y  +500 bps &  -0.017183846 &  -0.053239612 &                   0.080016435 &   0.040394763 &  -0.205695623 &  -0.234835612 \\
                    Fwd Start ATM 1y-10y  -100 bps &  -0.051882193 &  -0.026884683 &                   0.033386154 &   0.060631799 &   0.056462376 &   0.084316435 \\
                    Fwd Start ATM 1y-10y  -500 bps &  -0.086011918 &   0.013357459 &                  -0.013515854 &   0.093735342 &   0.352787554 &   0.499863495 \\
                             Zero Coupon ATM 20 yr &  -0.020559795 &   -0.00930056 &                   0.151888035 &   0.165129658 &  -0.010520053 &   0.000854595 \\
                      Zero Coupon ATM+100bps 20 yr &  -0.015250587 &  -0.014204215 &                   0.158132023 &   0.159362628 &  -0.083913572 &  -0.082940159 \\
                      Zero Coupon ATM+200bps 20 yr &  -0.010689903 &   -0.01836527 &                   0.163495696 &   0.154468945 &  -0.147184346 &  -0.153800747 \\
                      Zero Coupon ATM-100bps 20 yr &  -0.026816892 &  -0.003434873 &                   0.144529265 &   0.172028103 &   0.075632222 &   0.101475716 \\
                      Zero Coupon ATM-200bps 20 yr &  -0.036668124 &     0.0059908 &                   0.132943549 &   0.183113333 &   0.210477802 &   0.264081012 \\
\bottomrule
\end{tabular}


